A Sequent Calculus for Modelling Interferences

A logic calculus is presented that is a conservative extension of linear logic. The motivation beneath this work concerns lazy evaluation, true concurrency and interferences in proof search. The calculus includes two new connectives to deal with multisequent structures and has the cut-elimination property. Extensions are proposed that give first results concerning our objectives.

==> SECTIONS/PhaseSpace.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%			PHASE SEMANTICS
%\section{Phase semantics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		phase space (basic)

% \subsection{Phase space $\Mfock$}

In this section, a phase semantics is proposed for Linear Logic. It is built as a kind of Fock space on top of a free commutative monoid. Comultiplication is used to model the splitting process. We conjecture that it may give a phase semantics for our calculus. Let $(M,\star,1)$ be a free commutative, associative monoid with neutral element $1$. Elements range as $x, y, \dots$. The product will be denoted as a concatenation: $x y \triangleq x \star y$. We consider the following notations and definitions:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Construction of a symmetric Fock space $(\Mfock,\circ,+)$}


\begin{itemize}
\item $\Mronde{M}$ is the set of multisets of $M$. These multisets are denoted additively: $x_1 + \dots + x_n \triangleq \{x_1, \dots, x_n\}$. $M$ is considered as a subset of $\Mronde{M}$ by identifying a singleton and its element. The empty set may be denoted $0$.
\item $\Mcross{n}$ is the closure under $+$ of the cartesian product of $n$ copies of $\Mronde{M}$ (and $\times$ distributes over $+$). Elements range as $a, b, \dots$. Elements of the cartesian product of $M$ are called {\em simple}. $a_i$ is the $i$th part of the simple element $a$.
\item $\Msym{n}$ is the closure under $+$ of the symmetric cartesian product, i.e. $\Msym{n} = \Mcross{n} / {\mathfrak{S}}_n$ where ${\mathfrak{S}}_n$ is the group of permutations on $n$ elements. The symmetric product is denoted $\circ$.
\item $\Msym{0} = \Mcross{0} = \{\emptyset\}$.
\item $\Mfock = \bigcup_{n\geq 0} \Msym{n}$. Elements of $\Mfock$ range as $f, g, \dots$
\item Let $\Delta: \Mronde{M} \rightarrow \Mcross{2}$ be such that (shuffle coproduct on $\Mronde{M}$):
	$$\begin{array}{lrcl}
	\forall x\in M, & \Delta(x) & = & \sum_{x_{(1)}x_{(2)} = x} x_{(1)} \times x_{(2)} \\
	\forall a_1, a_2\in \Mronde{M}, & \Delta(a_1 + a_2) & = & \Delta(a_1) + \Delta(a_2)
	\end{array}$$
%	\item $\Delta(1) = 1 \circ 1$
	 We use the Sweedler notation: sums are over all possible decompositions.
\item $\Delta_{n-1}: \Mronde{M} \rightarrow \Mcross{n}$ ($n \geq 1$) is recursively defined:
	\begin{itemize}
	\item $\Delta_0 (a) = a$
	\item $\Delta_1 (a) = \Delta(a)$
	\item $\Delta_{n+1} (a) = (\Delta \times id^n)\circ \Delta_n(a)$ (here $\circ$ refers to composition and $id^n \triangleq id \times \dots \times id$ ($n$ times))
	\end{itemize}
\item We extend $\Delta_n$ as a morphism on $(\Mfock,\circ,+)$:
	\begin{itemize}
	\item $\Delta_n(f+g) = \Delta_n(f) + \Delta_n(g)$
	\item $\Delta_n(f \circ g) = \Delta_n(f) \circ \Delta_n(g)$
	\end{itemize} 
\end{itemize}

\begin{proposition}~
\begin{itemize}
\item $\Delta$ is coassociative and cocommutative.
\item $\forall n\geq 0, i\in [0,n],~ \Delta_{n+1} = (id^i \times \Delta \times id^{n-i}) \circ \Delta_{n}$ \hfill ($n$-coassociativity).
\item $\forall n\geq 0, i,j\in [1,n+1],~ c_{i,j} \circ \Delta_n = \Delta_n$ \hfill ($n$-cocommutativity) \\
where $c_{i,j}(a_1 \times \dots \times a_i \times \dots \times a_j \times \dots \times a_{n+1}) = a_1 \times \dots \times a_j \times \dots \times a_i \times \dots \times a_{n+1}$.
\end{itemize}
\end{proposition}
Proofs are obtained by direct computations and induction on $n$.
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \subsubsection{Extension of $\star$ as a product on $\Mfock$}
% 
We finally extend $\star$ to get a product on $\Mfock$:
\begin{definition}
Let $f\in \Msym{m}, g\in \Msym{n}$, $f$ and $g$ simple elements,
		$$ f \star g \triangleq \sum \circ_{i,j} f_{i(j)} g_{j(i)}$$
where $i \in [1,m]$ and $j \in [1,n]$.
$\star$ is extended by linearity to the Fock space.
\end{definition}
\begin{proposition}\label{starProp}\label{distrib_lemma} $\star$ enjoys the following properties:
\begin{itemize}
\item $\star$ is well defined on $\Mfock$ and is commutative, associative.
\item $\forall u \in M, \forall n\geq 0, i \in [0,n], \Delta_{n+1}(u) = \sum \Delta_i(u_{(1)})\circ \Delta_{n-i}(u_{(2)})$
\item $u \star (f \circ g) = \sum (u_{(1)} \star f) \circ (u_{(2)} \star g)$
\end{itemize}
\end{proposition}

\begin{proof}
Notations are the following ones:
$$
\left \{\begin{array}{lcl}
f & = & f_1 \circ \dots \circ f_m \\
f_i & = & f_{i(1)} \dots f_{i(n)} 
\end{array}\right.
~~~~
\left \{\begin{array}{lcl}
g & = & g_1 \circ \dots \circ g_n \\
g_j & = & g_{j(1)} \dots g_{j(m)} 
\end{array}\right.
$$
where $f_i$ and $g_j$ are elements of $M$. Then
$$f \star g = \sum f_{1(1)} g_{1(1)} \circ \dots \circ f_{1(n)} g_{n(1)} \circ f_{2(1)} g_{1(2)} \circ \dots \circ f_{m(n)} g_{n(m)} 
$$
\begin{itemize}
\item the definition does not depend on the chosen representatives: permuting $f_i$ with $f_j$ replaces in the sum the term $f_{i(k)}g_{k(i)}$ by $f_{j(k)}g_{k(i)}$ and $f_{j(l)}g_{l(j)}$ by $f_{i(l)}g_{l(j)}$. However, the sum being computed over all decompositions of $g_k$ and $g_l$, and invariant over permutations, the global sum remains the same. Finally, the product $\star$ is commutative as $\star$ is commutative on $M$.
\item Note that $f \star g$ is the symmetric of $\Delta_n(f) \cdot \Delta_m(g)$ where $\cdot$ is the dot product (here on $\Msym{mn}$).
\item The dot product is associative (because $\star$ is associative on $M$), so is the $\star$ product.
\item the two last propositions are proven by induction and direct computation.
\end{itemize}
\end{proof}

We add to $\Mronde{M}$ an element $\un$ and extend $\Delta$ in the following way: $\Delta(\un) = \un \times \un$. Note that $\un$ is neutral w.r.t. $\star$. $(\Mfock, \star, \circ, \un)$ is called a {\em distribution} space.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{The phase space is ($\Mfock, \leq, \perpfock, \un$)}
%
A model of Linear Logic may be obtained by defining as usual an order relation and by interpreting formulas of Linear Logic as facts. We use the following notations: $f,g \in \Mfock$, $F, G \subset \Mfock$. Elements of the dual are denoted with a prime: $f' \in F^\perp$. $A, B$ denote facts, i.e. subsets of $\Mfock$ closed by biorthogonal: $A = A^{\perp\perp}$. We give the following definitions:

\begin{definition}~
\begin{itemize}
\item $\geq$ is the least partial order relation on $\Mfock$ satisfying ($\forall f,g,h \in \Mfock$):
	\begin{description}
	\item[($\geq_1$)] $f \leq g$ then $f \star h \leq g \star h$
%	\item[($\geq_2$)] $f \leq g$ then $f \circ h \leq g \circ h$
	\item[($\geq_2$)] $f \leq f + g$
	\end{description}
\item $\perpfock$ is a subset of $\Mfock$ satisfying:
	\begin{description}
	\item[($\perpfock_1$)] it is the smallest ideal for $\geq$: $f \in \perpfock$ and $f \leq g$ then $g \in \perpfock$
	\item[($\perpfock_2$)] it contains a subset $\bot \subset M$
	\item[($\perpfock_3$)] $f,g \in \perpfock$ iff $f \circ g \in \perpfock$
%	\item[($\perpfock_4$)] $f\in\perpfock$ then $\exists f_1, f_2, f = f_1 \star f_2$ and $f_1 \circ f_2\in \perpfock$
	\end{description}
\item $f^\perp = \{g \in \Mfock / f\star g \in \perpfock\}$
\item $F^\perp = \bigcap_{f \in F} f^\perp$
\item $F \star G = \{f\star g / f\in F, g\in G \}$
\item $F \circ G = \{f\circ g / f\in F, g\in G \}$
\end{itemize}
\end{definition}

\begin{lemma}\label{order_lemma}
$$f < g \mbox{ then } \exists h\neq 0, \mbox{ such that } g = f + h$$
\end{lemma}
\begin{proof}
We proceed by induction on $p =m+n$: $f\in\Msym{m}$ and $g\in\Msym{n}$.
\begin{itemize}
\item The property is true for $p = m = n = 0$ ($f=g=0$ is the only possibility).
\item Let $p \geq 1$ and the property true for all $p' < p$. We consider the various cases implying $f<g$.
	\begin{description}
	\item[$(\geq_1)$ ] $\exists f_1, g_1, h_1$ such that $f= f_1 \star h_1$, $g = g_1 \star h_1$ and $f_1 < g_1$. Hence by induction (inductive construction of the partial order on $\Mronde{M}$ or induction on $p$), $\exists h_2\neq 0 \mbox{ such that } g_1 = f_1 + h_2$. Then $g = g_1 \star h_1 = (f_1 + h_2) \star h_1 = f_1 \star h_1 + h_2 \star h_1 = f + h_2 \star h_1$.
% 	\item[$(\geq_2)$ ] $\exists f_1, g_1, h_1$ such that $f= f_1 \circ h_1$, $g = g_1 \circ h_1$ and $f_1 < g_1$. Hence by induction (induction on $p$), $\exists h_2 \neq 0, n, \mbox{ st } g_1 = \Delta_n(f_1) + h_2$. Then $g = g_1 \circ h_1 = (\Delta_n(f_1) + h_2) \circ h_1 = \Delta_n(f_1)\circ h_1 + h_2 \circ h_1$. Suite ???
	\item[$(\geq_2)$ ] $g = f + h$: the case is obvious.
	\item[transitivity] $f_1 < f_2$ and $f_2 < f_3$. Then $\exists h_1\neq 0 \mbox{ such that } f_2 = f_1 + h_1$ and $\exists h_2\neq 0 \mbox{ such that } f_3 = f_2 + h_2$.Thus $f_3 = (f_1 + h_1) + h_2 = f_1 + (h_1 + h_2)$.
	\end{description}
\end{itemize}
\end{proof}

\begin{lemma}\label{choice_lemma}
$$f \in \perpfock \mbox{ iff } \exists (g_i)_{i\in I}, I \mbox{ finite non-empty}, g_i\in \perpfock, g_i \in M \mbox{ such that } f = \bigcirc_i g_i + h$$
\end{lemma}
\begin{proof}
One direction results from $(\perpfock_3)$, $(\geq_2)$. Suppose $f \in \perpfock$. We prove the other result by induction on $n$ such that $f\in \Msym{n}$.
\begin{itemize}
\item $n=1$ We can suppose that $f = \sum_{j\in J} f_j$ and $f_j\in M$. We proceed by induction on the cardinality of $J$. Either $f\in M$ and we are finished, or (definition of the order relation $\geq$) $\exists g\in\Mronde{M},g\in\perpfock, g\neq f$ such that $g < f$, hence $\exists h$ and $f = g+h$ (situation ($\perpfock_3$) does not occur). We finish by using the property on $g$.
\item Suppose the property true till $n-1$, $n>0$. Either situation $(\perpfock_1)$ occurs and $\exists g\in\Mronde{M},g\in\perpfock, g\neq f$ such that $g < f$ and we conclude with Lemma \ref{order_lemma}, or situation $(\perpfock_3)$ occurs and $\exists f_1,f_2$ and $f = f_1\circ f_2$ and $f_1,f_2\in \perpfock$ and induction on $n$ applies.
\end{itemize} 
\end{proof}

Note that Lemma~\ref{choice_lemma} shows in fact that the splitting of the context may be "anticipated" in terms of phase semantics (one element of a sum has a "good" property). Then the following property shows that the two sets of connectives coincide:
 
\begin{proposition}
$(A \star B) ^{\perp\perp} = (A^\perp \circ B^\perp)^\perp$ (i.e. $\otimes$ and $\cpar$ are equivalent) when $A$ and $B$ are facts.
\end{proposition}

\begin{proof}
\begin{itemize}
\item $A^\perp \circ B^\perp \subset (A \star B)^\perp$: with the definition given,
	\begin{eqnarray*}
	(A^\perp \circ B^\perp) \star A \star B & = & ((A^\perp \star A) \circ B^\perp + A^\perp \circ (B^\perp \star A))  \star B \\
	& = & (A^\perp \star A) \circ (B^\perp \star B) + (A^\perp \star A \star B) \circ B^\perp \\
	&  &	+ (A^\perp \star B) \circ (B^\perp \star A) + A^\perp \circ (B^\perp \star A \star B) 
	\end{eqnarray*}
	and $(A^\perp \star A) \circ (B^\perp \star B) \subset \bot$ hence the result follows.
\item $(A \star B)^\perp \subset (A^\perp \circ B^\perp)^{\perp\perp}$:
	\begin{itemize}
	\item let $u \in (A^\perp \circ B^\perp)^{\perp}$, then $\forall a'\in A^\perp, b' \in B^\perp$, $u \star (a' \circ b') \in \bot$. 
	\item Furthermore $u \star (a' \circ b') = \sum (u_{(1)} \star a') \circ (u_{(2)} \star b')$ (Lemma~\ref{distrib_lemma}). 
	\item Then by Lemma~\ref{choice_lemma}, there exist $u_{(1)}$ and $u_{(2)}$ such that $u=u_{(1)} \star u_{(2)}$, and $(u_{(1)} \star a') \circ (u_{(2)} \star b') \in \bot$.
	\item Hence $u_{(1)} \star a' \in \bot$ and $u_{(2)} \star b' \in \bot$, i.e. $u_{(1)} \in a'^\perp$ and $u_{(2)} \in b'^\perp$, then $u=u_{(1)} \star u_{(2)} \in a'^\perp \star b'^\perp$.
	\item Then $u \in \bigcap_{a',b'} a'^\perp \star b'^\perp = \bigcap_{a'} a'^\perp \star \bigcap_{b'} b'^\perp$.
	\item Furthermore $A^\perp = \bigcup_{a'} \{a'\}$, then $A = A^{\perp\perp} = \bigcap_{a'} a'^\perp$, idem for $B$.
	\item Then $u \in A \star B$.
	\end{itemize}
\end{itemize}
\end{proof}


\begin{definition}
A {\em phase structure} $(P,\mathcal V)$ is given by a phase space $P$ and a valuation that associates a fact $\mathcal{V}(p)$ to each proposition symbol $p$.
The interpretation $\mathcal{V}(A)$ of a formula $A$ is defined in a standard way:
$$\begin{array}{lclclcl}
\multicolumn{7}{c}{\mathcal{V}(A^\perp) = \mathcal{V}(A)^\perp}\\
\mathcal{V}(\perp) & = & \un &~~~~& \mathcal{V}(\un) & = & \perp \\
\mathcal{V}(A\otimes B) & = & \mathcal{V}(A) \otimes \mathcal{V}(B) && \mathcal{V}(A\Par B) & = & \mathcal{V}(A) \Par \mathcal{V}(B)\\
\mathcal{V}(A\ctimes B) & = & \mathcal{V}(A) \ctimes \mathcal{V}(B) && \mathcal{V}(A\cpar B) & = & \mathcal{V}(A) \cpar \mathcal{V}(B)\\
\mathcal{V}(A\oplus B) & = & \mathcal{V}(A) \oplus \mathcal{V}(B) && \mathcal{V}(A\with B) & = & \mathcal{V}(A) \with \mathcal{V}(B)
\end{array}
$$

The interpretation of sequents is defined in the following way: let $\mathcal S$ be a multisequent, $\mathcal S$  may be defined as a triple $(I,\mathcal{O},p)$ where $I\subset\mathbb{N}$ is finite, $\mathcal{O}$ is a finite multiset of occurrences of formulas, $p$ is a function from $I$ to the powerset of $\mathcal{O}$ (i.e. $p(i)$ gives the set of occurrences present in the $i^{th}$ sequent of $\mathcal S$). Define $n(A,i) = \#\{j\leq i / A \in p(j)\}$. Then
$$ \mathcal{V}(\mathcal{S}) 
	= \{ \sum \bigcircop_{i\in I} 
			\bigstarop_{\substack{X\in p(i) \\ x'\in \mathcal{V}(X^\perp)}} 
				x'_{(n(X,i))}\}^{\perp\perp}$$
where the sum is over all tuples $(x'_{(1)},\dots,x'_{(n(X,|I|))})$ for all $X^\perp$, i.e. $x'\in \mathcal{V}(X^\perp)$ and $\Delta_{n(X,|I|)}(x') = \sum_{x' = x'_{(1)} \star \dots \star x'_{(n(X,|I|))}} x'_{(1)}\circ \dots \circ x'_{(n(X,|I|))}$.
\end{definition}

% \begin{example}
% \begin{itemize}
% \item $\{A,B\}$ (i.e. $\vdash A,B$) has the following denotation:
% $$\{ a'\star b' / a'\in\mathcal{V}(A)^\perp, b'\in\mathcal{V}(B)^\perp\}^{\perp\perp}$$
% \item $\{A,B\}\{B,C\}\{C,D\}$ (i.e. $\vdash A, B ~~~ \vdash B,C ~~~ \vdash C,D$) has the following denotation (this multisequent involves only 4 occurences of formulas !):
% $$\{ \sum (a'\star b'_{(1)}) \circ (b'_{(2)}\star c'_{(2)}) \circ (c'_{(1)}\star d')\}^{\perp\perp}$$
% where the sum is over triples of elements $a'\in A^\perp, b'\in B^\perp, c'\in C^\perp$ and, the triple being fixed, the sum ranges over all pairs $(b'_{(1)}, b'_{(2)})$ and $(c'_{(1)}, c'_{(2)})$ where $\Delta(b') = \sum b'_{(1)} \circ b'_{(2)}$ and $\Delta(c') = \sum c'_{(1)} \circ c'_{(2)}$.
% Note that, thanks to Lemma \ref{distrib_lemma}, the denotation may also be written:
% $$\{ \sum ((a'\circ c'_{(2)}) \star b') \circ (c'_{(1)}\star d')\}^{\perp\perp}$$
% or
% $$\{ \sum (a'\star b'_{(1)}) \circ ((b'_{(2)} \circ  d') \star c')\}^{\perp\perp}$$
% However there is no possibility to give a denotation without reference to a sum (i.e. the structure is not well parenthesized).
% \end{itemize}
% \end{example}

Note that the valuation $\mathcal{V}$ is well defined as $\Delta_n$ is associative for all $n$, and operations $\circ, \star$ are associative and commutative.

% By convention, we note:
% \begin{itemize}
% \item $\alpha$ (resp. $\beta$, $\gamma$, ...) an element of $A$ (resp. $B$, $\Gamma$, ...),
% \item $a$ (resp. $b$, $g$, ...) a monomial of $\alpha$ (resp. $\beta$, $\gamma$, ...),
% \item $\alpha'$ (resp. $\alpha''$) an element of $A^\perp$ (resp. $A^{\perp\perp}$).
% \end{itemize}

\begin{definition}
Let $A$ be a formula, $A$ is {\em valid for $\mathcal{V}$} iff $\mathcal{V}(A) \subset \perpfock$. A multisequent $\mathcal{S}$ is {\em valid} iff $\mathcal{V}(\mathcal{S}) \subset \perpfock$ for all phase structure $(P,\mathcal{V})$.
\end{definition}

\begin{theorem}\label{validity}
If a multisequent is provable in Linear Logic, then it is valid.
\end{theorem}
The proof is done, as usual, by induction on the structure of a proof.

Even if the phase semantics as described here has lost part of its significance w.r.t. \CMALL\ because of Lemma~\ref{choice_lemma}, we conjecture that this algebraic framework may give fruitful insights to the understanding of calculi over multisequents.


==> SECTIONS/csInterf.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{CLL with Interferences}

Connectives $\cpar$ and $\ctimes$ as defined in Sect.~\ref{sec:calculus} cannot deal with interference. In fact, the calculus is designed having lazy logic programming in mind: the context is not immediately split with the $\ctimes$ rule but a splitting should occur when applying $\cpar$ rules. However, even if a splitting property should be valid, there is no need to have it explicitly for one of the connectives. In fact, interference may be introduced by considering triples instead of pairs of hypotheses in the rule introducing $\cpar$. We then modify the calculus given for \CMALL\ by changing the rules for connectives $\ctimes$ and $\cpar$ (we call this calculus I-CLL):

$$
\scriptInfer[(\ctimes)]{\dots \{\Gamma_i, A\ctimes B\}
                        \{\Gamma_i, \Delta_j, A\ctimes B\}
                        \{\Delta_j, A\ctimes B\} 
                 \dots}
      {\dots \{\Gamma_i, A\} \dots
	  &
	   \scriptstyle \dots \{\Delta_j, B\} \dots}
\hspace{2cm}
\scriptInfer[(\cpar)]{\dots \{\Gamma_i, A\cpar B\} \dots}
     {\dots \{\Gamma_i, A\} \{\Gamma_i, A, B\} \{\Gamma_i,B\} \dots}
$$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Provable and unprovable sequents}


It is easy to prove that $\cpar$ is asynchronous and $\ctimes$ is synchronous, and also that cut-elimination is valid.
Note that the calculus \CMALL\ can be simulated by I-CLL (in order to distinguish the two connectives we note $\cpar\cpar$ connective cpar defined in \CMALL\ and $\cpar$
the connective defined in I-CLL):
\begin{proposition}
If ${\mathcal S}[A\cpar\cpar B]$ is provable in \CMALL\ then ${\mathcal S}[A\cpar B]$ is provable in I-CLL.
\end{proposition}
\begin{proof}
The following partial proof shows that one can use a
proof with $\cpar\cpar$ to build a proof with $\cpar$. Remind that these connectives are asynchronous.

$$
\scriptInfer[\cpar]{\dots \{\Gamma_i, A\cpar B\} \dots}
      {\scriptInfer[d]{\dots \{\Gamma_i, A\} 
                       \{\Gamma_i, A, B\} 
                       \{\Gamma_i, B\} \dots}
             {\scriptInfer[w]{\dots \{\Gamma_i, A\} 
                              \{\Gamma_i, A\} 
                              \{\Gamma_i, B\} \dots}
                    {\dots \{\Gamma_i, A\} 
                           \{\Gamma_i, B\} \dots}
      }      }
$$
\end{proof}

This allows us to recover previous properties: $A\otimes B \la A\cpar B$ and $\otimes \not\equiv ~\cpar$. We are now able to model independent actions:

\begin{example}
Suppose we have two 'packs' of actions: $f = \bigoplus f_n$ (resp. $g = \bigoplus g_n$) such that $f_n$ (resp. $g_n$) transforms $n$ occurences of $a$ (resp. $b$) into $n$ occurences of $a$ and $n$ occurences of $b$, where $n\geq 1$. Suppose also that we have only one resource
of each kind (hence one $a$ and one $b$).
We want to simulate the two following situations: 
\begin{itemize}
\item[(i)] if the two actions are applied (whatever may be the order) then we have three possible results:
3 $a$ and 2 $b$, 2 $a$ and 3 $b$, 2 $a$ and 2 $b$. The first (resp. second) result is obtained when action $f$ (resp. $g$) is applied first followed by action $g$ (resp. $f$). The third result occurs when the two actions are performed simultaneously.
\item[(ii)] if the two actions are applied concurrently, there is only one possible result: we get 2 $a$ and 2 $b$.
\end{itemize}

As proofs are one-sided (and on the right), we take the negation of propositional variables to get more readable proofs.
Let us formalize $f_1$ as $a^\perp \la 0\ctimes((a^\perp\otimes b^\perp) \with (\bot\cpar(a^\perp\otimes b^\perp)))$ and
$g_1$ as $b^\perp \la 0\ctimes((a^\perp\otimes b^\perp) \with (\bot\cpar(a^\perp\otimes b^\perp)))$. These formalizations are straightforwardly generalized to $f_n$ and $g_n$.

We consider the following aliases: $X \equiv \top\cpar Y$ and $Y \equiv (a\Par b) \plus (1\ctimes(a\Par b))$. Hence 
$f^\perp \equiv a^\perp\otimes X$ and $g^\perp \equiv b^\perp\otimes X$.
Notice that we omit $\oplus$ rules in proofs to shorten them and recall that when two occurences of the same formula appear, these occurences are indexed.

\begin{itemize}
\item[(i)] application of $f$ and $g$ is formalized as $f\otimes g$:
$$
\scriptInfer[\Par]{\{a, b, f^\perp\Par g^\perp\}}
      {\scriptInfer[\otimes]{\{a, b, f^\perp, g^\perp\}}
             {\{a^\perp, a\}
              &
              \scriptInfer[\cpar]{\{b, X, g^\perp\}}
                    {\scriptInfer[d]{\{b, \top, g^\perp\}
                               \{b, \top, Y, g^\perp\}
                               \{b, Y, g^\perp\}}
                           {\scriptInfer[\top]{\{b, \top, g^\perp\}
                                         \{b, \top, Y, g^\perp\}
                                         \{b, Y, g^\perp\}}
                                  {\scriptInfer[\Par]{\{b, Y, g^\perp\}}
                                         {\infer*[]{\scriptstyle \{b, a, b, g^\perp\}}
                                                {\scriptstyle \{2a, 3b\}}
      }      }      }      }      }      }
$$
The other results are obtained by swapping $f$ and $g$ or by using $g$ only on one $b$ in the last step
of the previous proof.
\item[(ii)] concurrent application of $f$ and $g$ is formalized as $f\ctimes g$.
$$
\scriptInfer[\cpar]{\{a, b, f^\perp\cpar g^\perp\}}
      {\scriptInfer[d]{\{a, b, f^\perp\}
                 \{a, b, f^\perp, g^\perp\}
                 \{a, b, g^\perp\}}
            {\scriptInfer[d]{\{a, b, f^\perp\}
                       \{a, b, f^\perp, g^\perp\}
                       \{b, g^\perp\}}
                   {\scriptInfer[\otimes]{\{a, f^\perp\}
                                    \{a, b^\perp, f^\perp, g^\perp\}
                                    \{b, g^\perp\}}
                          {\scriptInfer[ax]{\{a^\perp, a\}}{}
                           &
                           \scriptInfer[\otimes]{\{X_1\}
                                           \{X_1, b, g^\perp\}
                                           \{b, g^\perp\}}
                                 {\scriptInfer[\cpar]{\{X_1\}
                                                \{X_1, X_2\}
                                                \{X_2\}}
                                        {\scriptInfer[d]{\{\top\}
                                                   \{\top, Y\}
                                                   \{Y\}
                                                   \{\top, X_2\}
                                                   \{\top, Y, X_2\}
                                                   \{Y, X_2\}
                                                   \{X_2\}}
                                              {\scriptInfer[d]{\{\top\}
                                                         \{\top\}
                                                         \{Y\}
                                                         \{\top, X_2\}
                                                         \{\top, Y, X_2\}
                                                         \{Y, X_2\}
                                                         \{X_2\}}
                                                     {\scriptInfer[\top]{\{\top\}
                                                                   \{\top\}
                                                                   \{Y\}
                                                                   \{\top, X_2\}
                                                                   \{Y, X_2\}
                                                                   \{Y, X_2\}
                                                                   \{X_2\}}
                                                            {\scriptInfer[\ctimes]{\{Y\}
                                                                             \{Y, X_2\}
                                                                             \{Y, X_2\}
                                                                             \{X_2\}}
                                                                   {\scriptInfer[1]{1}{}
                                                                    &
                                                                    \scriptInfer[\Par]{\{a\Par b, X_2\}
                                                                                 \{X_2\}}
                                                                         {\infer*[]{\scriptstyle \{a, b, X_2\}
                                                                                    \{X_2\}}
                                                                               {\scriptstyle \{2a,2b\}}
                                  }}}}}}
                                  &
                                  \scriptInfer[ax]{\{b^\perp, b\}}{}
}}}}}
$$
Note that the sequent $\{a, b, f^\perp\cpar g^\perp\}$ is not provable when using $\{2a, 3b\}$ as hypothesis.
\end{itemize}
\end{example}

